Fluctuation Effects on the Physical Properties of Cd2Re2O7 Near 200 K

Experimental investigation of the resistivity $\rho$, susceptibility $\chi$, specific heat C$_p$, and Hall coefficient R$_H$ of the pyrochlore Cd$_2$Re$_2$O$_7$ reveals the presence of a continuous phase transition of uncertain origin with critical temperature T* = 200 K. Electron and X-ray diffraction measurements indicate that a commensurate structural transformation accompanies the changes in the electronic properties, implying that lattice as well as electronic degrees of freedom are involved in the transition. Remarkable scaling relationships between $\rho$, $\chi$, and C$_p$ are observed, indicating that fluctuations are crucial in the transition regime. Scenarios involving both spin and ionic density fluctuations are considered in the evaluation of the data. Although the observed structural transition suggests that ionic density fluctuations are likely to be important, a scaling relationship between $\rho$ and $\chi$ over a wide temperature range suggests that spin fluctuations may be playing a role as well.

==> Cd2Re2O7IIbib.tex <==
@ARTICLE{mandrus,
   author = "D. Mandrus and J.R. Thompson and R. Gaal and L. Forro and C.J. Bryan and B.C. Chakoumakos and L.M. Woods and B.C. Sales and R.S. Fishman and V. Keppens",
   year = "2001",
   journal = "Phys. Rev. B",
   volume = "63",
   pages = "195104"
}

@ARTICLE{hanawa,
   author = "{M. Hanawa {\it et al.}}",
   year = "2001",
  journal = "cond-mat/0106421" }

 @ARTICLE{subr,
    author = "{For a review, see M.A. Subramanian and G. Aravamudan and G.V. Subba
Rao}",
    year = "1983",
    journal = "Prog. Solid State Chem.",
   volume = "15",
   pages = "55"
}

 @ARTICLE{donohue,
   author = "P.C. Donohue and J.M. Longo and R.D. Rosenstein and L. Katz",
   year = "1965",
   journal = "Inorg. Chem.",
   volume = "4",
   pages = "1152"
}

@ARTICLE{he,
   author = "{J. He {\it et al.}}",
   year = "2001",
  journal = "(to be submitted)" }

@ARTICLE{jin,
    author = "R. Jin and J. He and S. McCall and C.S. Alexander and F. Drymiotis and D. Mandrus",
    year = "2001",
    journal = "Phys. Rev. B",
   volume = "64",
   pages = "R15138"
}


@ARTICLE{moriya,
   author = "T. Moriya and A. Kawabata",
   year = "1973",
   journal = "J. Phys. Soc. Jpn.",
   volume = "34",
   pages = "639"
  journal = "\bf {ibid}",
   volume = "35",
   pages = "669"}

@ARTICLE{singh,
    author = "{D.J. Singh and P. Blaha and K. Schwarz and J.O. Sofo}",
    year = "2001",
    journal = "cond-mat/0108226"
}


 @ARTICLE{black,
   author = "{K. Blacklock and H.W. White}",
   year = "1979",
   journal = "J. Chem. Phys.",
   volume = "71",
   pages = "5287"
}
 @ARTICLE{chandra,
   author = "P.Chandra",
   year = "1989",
   journal = "J. Phys.: Condens. Matter",
   volume = "1",
   pages = "10067"
}

@ARTICLE{bucher,
   author = "{B. Bucher and P. Steiner and J. Karpinski and E. Kaldis and P. Wachter}",
   year = "1993",
   journal = "Phys. Rev. Lett.",
   volume = "70",
   pages = "2012"
}

@ARTICLE{wang,
    author = "R. Wang and A.W. Sleight",
    year = "1998",
    journal = "Mater. Res. Bull.",
  volume = "33",
   pages = "1005"
}

@ARTICLE{fujimoto,
    author = "{S. Fujimoto}",
    year = "2001",
    journal = "cond-mat/0103430"
}

@ARTICLE{fisher,
   author = "{M.E. Fisher and J.S. Langer}",
   year = "1968",
   journal = "Phys. Rev. Lett.",
   volume = "20",
   pages = "665"
}

@ARTICLE{fisher2,
   author = "{M.E. Fisher}",
   year = "1962",
   journal = "Philos. Mag.",
   volume = "7",
   pages = "1731"
}
 @ARTICLE{takimoto,
   author = "T. Takimoto and T. Moriya",
   year = "1996",
   journal = "Solid State Commun.",
   volume = "99",
   pages = "457"
}

@ARTICLE{whh,
   author = "N.R. Werthamer and E. Helfand and P.C. Hohenberg",
   year = "1966",
   journal = "Phys. Rev.",
   volume = "147",
   pages = "295"
}

@ARTICLE{kondo,
   author = "S. Kondo and D.C. Johnston and C.A. Swenson {\it et al.} ",
   year = "1997",
   journal = "Phys. Rev. Lett.",
   volume = "78",
   pages = "3729"
}

@ARTICLE{kwok,
   author = "R.S. Kwok and G. Gruner and S.E. Brown ",
   year = "1990",
   journal = "Phys. Rev. Lett.",
   volume = "65",
   pages = "365"

}

@ARTICLE{fleming,
   author = "R.M. Fleming and F.J. DiSalvo and R.J. Cava and J.W. Waszczak ",
   year = "1981",
   journal = "Phys. Rev. B",
   volume = "24",
   pages = "2850"

}

@ARTICLE{rice,
   author = "T.M. Rice and G.K. Scott",
   year = "1975",
   journal = "Phys. Rev. Lett.",
   volume = "35",
   pages = "120"

}
 @ARTICLE{chako,
   author = "{B. Chakoumakos {\it et al.}}",
   year = "2001",
   journal = "(to be submitted)",
}

 @ARTICLE{gaulin,
   author = "{B.D. Gaulin}",
 year = "2001",
   journal = "(private communication)",
}

 @ARTICLE{fang,
   author = "{Z. Fang}",
 year = "2001",
   journal = "(private communication)",
}

@ARTICLE{bhatt,
   author = "R.N. Bhatt",
   year = "1977",
   journal = "Phys. Rev. B",
   volume = "16",
   pages = "1915"

}

